DreamCraft3D++: Efficient Hierarchical 3D Generation with Multi-Plane Reconstruction Model

We introduce DreamCraft3D++, an extension of DreamCraft3D that enables efficient high-quality generation of complex 3D assets. DreamCraft3D++ inherits the multi-stage generation process of DreamCraft3D, but replaces the time-consuming geometry sculpting optimization with a feed-forward multi-plane based reconstruction model, speeding up the process by 1000x. For texture refinement, we propose a training-free IP-Adapter module that is conditioned on the enhanced multi-view images to enhance texture and geometry consistency, providing a 4x faster alternative to DreamCraft3D's DreamBooth fine-tuning. Experiments on diverse datasets demonstrate DreamCraft3D++'s ability to generate creative 3D assets with intricate geometry and realistic 360{\deg} textures, outperforming state-of-the-art image-to-3D methods in quality and speed. The full implementation will be open-sourced to enable new possibilities in 3D content creation.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> sections/method.tex <==
% \section{Preliminaries}
% DreamFusion~\cite{poole2022dreamfusion} achieves text-to-3D generation by utilizing a pretrained text-to-image diffusion model $\bm{\epsilon}_\phi$ as an image prior to optimizing the 3D representation parameterized by $\theta$. 

% The image $\bm{x}=g(\theta)$, rendered at random viewpoints by a volumetric renderer, is expected to represent a sample drawn from the text-conditioned image distribution $p(\bm{x}|y)$ modeled by a pretrained diffusion model. The diffusion model $\phi$ is trained to predict the sampled noise $\bm{\epsilon}_\phi(\bm{x}_t;y,t)$ of the noisy image $\bm{x}_t$ at the noise level $t$, conditioned on the text prompt $y$. A \emph{score distillation sampling} (SDS) loss encourages the rendered images to match the distribution modeled by the diffusion model. Specifically, the SDS loss computes the gradient:
% \begin{equation}
% \nabla_{\theta}\mathcal{L}_\textnormal{SDS}(\phi, g(\theta))=\mathbb{E}_{t, \bm{\epsilon}}\Big[\omega(t)(\bm{\epsilon}_{\phi}(\bm{x}_{t};y,t)-\bm{\epsilon})\frac{\partial \bm{x}}{\partial \theta}\Big],
% \label{eq:sds}
% \end{equation}
% which is the per-pixel difference between the predicted and the added noise upon the rendered image, where $\omega(t)$ is the weighting function. 

% One way to improve the generation quality of a conditional diffusion model is to use the classifier-free guidance (CFG) technique to steer the sampling slightly away from the unconditional sampling, \ie,  $\epsilon_\phi(\bm{x}_t;y,t) + \omega\epsilon_\phi(\bm{x}_t;y,t) - \omega\epsilon_\phi(\bm{x}_t,t,\varnothing)$, where $\varnothing$ represents the ``empty'' text prompt. Typically, the SDS loss requires a large CFG guidance weight for high-quality text-to-3D generation, yet this will bring side effects like over-saturation and over-smoothing~\cite{poole2022dreamfusion}. 

% Recently, Wang et al. ~\cite{wang2023prolificdreamer} proposed a variational score distillation (VSD) loss that is friendly to standard CFG guidance strength and better resolves unnatural textures. Instead of seeking a single data point, this approach regards the solution corresponding to a text prompt as a random variable. Specifically, VSD optimizes a distribution  $q^{\mu}(\bm{x}_0|y)$ of the possible 3D representations $\mu(\theta|y)$ corresponding to the text $y$, to be closely aligned with the distribution defined by the diffusion timestep $t=0$, $p(\bm{x}_0|y)$, in terms of KL divergence:
% \begin{equation}
% \mathcal{L}_\textnormal{VSD} = D_\textnormal{KL}(q^{\mu}(\bm{x}_0|y) || p(\bm{x}_0|y)).
% \end{equation}
% \cite{wang2023prolificdreamer} further shows that this objective can be optimized by matching the score of noisy real images and that of noisy rendered images at each time $t$, so the gradient of $\mathcal{L}_\textnormal{VSD}$ is
% \begin{equation}
% \scalebox{0.8}{$
% \nabla_{\theta}\mathcal{L}_\textnormal{VSD}(\phi, g(\theta))=\mathbb{E}_{t, \bm{\epsilon}}\Big[\omega(t)(\bm{\epsilon}_{\phi}(\bm{x}_{t};y,t)-\bm{\epsilon}_\textnormal{lora}(\bm{x}_{t};y,t,c))\frac{\partial \bm{x}}{\partial \theta}\Big].
% $}
% \label{eq:vsd}
% \end{equation}
% Here, $\bm{\epsilon}_\textnormal{lora}$ estimates the score of the rendered images using a LoRA (Low-rank adaptation)~\cite{hu2021lora} model. The obtained variational distribution yields samples with high-fidelity textures. However, this loss is applied for texture enhancement and is helpless to the coarse geometry initially learned by SDS. Moreover, both the SDS and VSD attempt to distill from a fixed target 2D distribution which only assures per-view plausibility rather than a global 3D consistency. Consequently, they suffer from the same appearance and semantic shift issue that hampers the perceived 3D quality.


% \section{DreamCraft3D: Overview}
% % We propose a hierarchical pipeline for 3D content generation as illustrated in Figure~\ref{fig:diagram}. Our method first leverages a state-of-the-art text-to-image generative model to generate a high-quality 2D image from a text prompt. In this way, we can leverage the full power of state-of-the-art 2D diffusion models to depict intricate visual semantics described in the text, retaining the creative freedom of 2D models. We then lift this image to 3D through cascaded stages of geometric sculpting and texture boosting. By decomposing the problem, we can apply specialized techniques at each stage. For geometry, we prioritize multi-view consistency and global 3D structure, allowing for some compromise on detailed textures. With the geometry fixed, we then focus solely on optimizing realistic and coherent texture, for which we jointly learn a 3D-aware diffusion prior that bootstraps the 3D optimization. Next, we elaborate on key design considerations for the two phases. 

% We propose a hierarchical pipeline for high-quality and efficient 3D content generation as illustrated in Figure~\ref{fig:diagram}. Given a single image, our method first leverages state-of-the-art multi-view diffusion models to produce several orthogonal and consistent multi-view images. Then, we build a feed-forward sparse-view 3D reconstruction model to efficiently infer the underlying textured meshes from those input images. For this stage, we prioritize multi-view consistency and global 3D structure, allowing for some compromise on detailed textures and geometry. Finally, we focus on jointly optimizing realistic and coherent texture as well as detailed geometry, with a training-free object-aware diffusion prior.


% \begin{figure}[t]
% \begin{center}
% %\framebox[4.0in]{$\;$}
% \begin{overpic}[width=\linewidth]{Images/diagram.pdf}
% \put(72,28){\footnotesize $\mathcal{L}_\textnormal{BSD}$}
% \put(70,61){\footnotesize $\mathcal{L}_\textnormal{SDS},\mathcal{L}_\textnormal{3D-SDS}$}
% \end{overpic}
% \end{center}
% \caption{DreamCraft3D leverages a 2D image generated from the text prompt and uses it to guide the stages of geometry sculpting and texture boosting. When sculpting the geometry, the view-conditioned diffusion model provides crucial 3D guidance to ensure geometric consistency. We then dedicately improve the texture quality by conducting a cyclic optimization. We augment the multi-view renderings and use them to finetune a diffusion model, DreamBooth, to offer multi-view consistent gradients to optimize the scene. We term the loss that distills from an evolving diffusion prior as bootstrapped distillation sampling ($\mathcal{L}_\textnormal{BSD}$ in the figure). 
% }
% \vspace{-1.0em}
% \label{fig:diagram}
% \end{figure}


% \section{Dream MP-LRM: Multiplane-based large reconstruction model}

% We now introduce the detailed architecture of the multiplane-based large reconstruction model (MP-LRM). As outlined in Fig. 2, given the input multi-view images and normal maps with known camera poses, a convolutional U-Net is used to map the input images along with the normal maps to a set of nonorthogonal multiple planes. Then we use lightweight multi-layer perceptions (MLPs) to decode the triplane features into SDF values, texture color and Flexicubes parameters. Lastly, these values are used to get texture mesh by dual marching cubes. Below, we explain the key components of MP-LRM in detail.

% \subsection{Nonorthogonal multi-plane representation with U-Net based backbone} 
% At the core of our framework is to a U-Net based backbone to predict Nonorthogonal multi-plane representation from multi-view images. The network architecture is shown in Figure 3. We take multi-view images and the corresponding normal maps with known poses as the input. Following previous works [57], we use the Plücker ray embedding to densely encode the camera poses. The RGB value and ray embedding are concatenated into a 12-channel feature map and then feed through a U-Net based backbone to predict a set of nonorthogonal planes. "Nonorthogonal" means the planes are not axis-aligned as the triplanes used in other methods. We use nonorthogonal planes instead of orthogonal axis-aligned planes because we think it is inefficient to learn the mapping from 2D posed image to the orthogonal plane features. If the network capacity is not large enough, the mapping result is prone to blurry. Considering that multi-view diffusion models always generate fix-viewed images, we can let the network focus on learning pixel-algined feature without learning to unpose them in space. Here we use a convolutional U-Net to learn the mapping from 2D posed image to the nonorthogonal plane features. Compared to transformer-based methods [18, 21, 63, 70], our U-shape design has a larger bandwidth in preserving the input information, leading to highly detailed triplane features and finally elaborate textured meshes. Moreover, the convolutional network fully utilizes the geometry prior of the spatial correspondance of triplanes and input six orthograhic images, which greatly fasten the convergence and stabilize the training. Our model can get reasonable reconstruction results at very early stage of training (around 20 minutes of training from scratch). Also, our model can be trained with a much smaller batch size 32 (compared to transformer-based LRM that uses a batch size of 1024), which makes that all of our experiments can be conducted on an 8-GPU-cards machine. The overall training cost of our reconstruction model is only 1/8 than LRM. More details are shown in the experiments (see Sec. 4.1).


% \subsection{Learnable plane embeddings} 
% Since the generated multi-view images are always within small elevation range, we don't have enough information of top and bottom views. Therefore, the meshes are prone to holes or artifacts at top and bottom views. To complement top and bottom view information, we set two additional learnable plane embeddings placed at the top and bottom respectively and feed through the U-Net based backbone. Our experiments prove that this will dilivate holes clearly. 

% \subsection{Decoding planes to flexicubes} 
% Previous generic 3D generation methods mostly adopt NeRF [35] or Gaussian splatting [19] as the geometry representation, which relies on extra procedures like Marching Cubes (MC) to extract the iso-surface, suffering from topological ambiguities and struggling to represent high-fidelity geometric details. In this work, we use Flexicubes [46] as our geometry representation. It can get meshes from the features on the grid by dual marching cubes [36] during training. The features include SDF values, deformation and weights. The texture is obtained by querying the color at the surface. Flexicubes enables us to train our reconstruction model with textured mesh as the final output in an end-to-end manner. Given the surface vertices, we project them into each nonorthogonal plane and query the feature by bilinear sampling. The features from all planes are aggregated by channel-wise concatenation.  

% \subsection{Loss Function}
% \noindent\textbf{RGB loss.}
% During training, we render the images at the $M$ supervision views using the predicted Gaussian splats, and minimize the image reconstruction loss. Let ${I_{i'}^|i' = 1, 2, ..., M}$ be the set of groundtruth views, and ${\hat{I}_i^}$ be the rendered images, our loss function is a combination of MSE (Mean Squared Error) loss and Perceptual loss:
% \begin{equation}
% \mathcal{L} = \frac{1}{M} \sum_{i'=1}^M \left( \text{MSE}(\hat{I}_i^, I_i^) + \lambda \cdot \text{Perceptual}(\hat{I}_i^, I_i^) \right),
% \label{eq:loss}
% \end{equation}
% where $\lambda$ is the weight of the perceptual loss. We empirically find that the perceptual loss in based on VGG-19 network provides a more stable training than LPIPS used in [27,32,63,68], and we use it in this work.

% \noindent\textbf{Depth and normal loss.} 
% In addition, akin to~\citep{deng2023nerdi}, we fully exploit the geometry prior inferred from the reference image, and enforce the consistency with the depth and normal map computed for the reference view. The corresponding  depth and normal loss are respectively computed as:
% \begin{equation}
%     \mathcal{L}_\textnormal{depth}= -\frac{\text{conv}(\bm{d},\hat{\bm{d}})}{\sigma(\bm{d}) \sigma(\hat{\bm{d}})},
%     \quad \mathcal{L}_\textnormal{normal}= -\frac{\bm{n} \cdot \hat{\bm{n}}}{{\Vert \bm{n} \Vert}_2 \cdot {\Vert \hat{\bm{n}} \Vert}_2},
% \end{equation}
% where $\text{conv}(\cdot)$ and $\sigma(\cdot)$ represent the covariance and variance operators respectively. The depth loss adopts the form of negative Pearson correlation $\mathcal{L}_\textnormal{depth}$ to account for the scale mismatch in depth.


% \noindent\textbf{GAN loss.} Generative adversarial networks (GANs) have proven to be a powerful framework for training large generative models to synthesize realistic images. While it is easy to optimize pixel-wise losses like mean squared error (MSE) between the reconstructed and ground truth images, pixel-wise losses tend to produce blurry results that lack high-frequency details. In contrast, the adversarial loss from a GAN discriminator can capture higher-order image statistics and encourage the generator to produce sharper, more realistic reconstructions. 

% Specifically, the reconstructor is set as the generator, and we initialize a multi-layer discriminator. During training, we alternate between optimize the generator and discriminator networks based on the standard non-saturation GAN loss as below:

% \begin{equation}
%     \begin{aligned}
%         \mathcal{L}_{total} &= \mathcal{L}_{recon} + \lambda_G \mathcal{L}_G \\
%         &+ \lambda_D \Big(\mathbb{E}_{x \sim p_{data}(x)}[\max(0, 1 - D(x))] \\
%         &+ \mathbb{E}_{z \sim p(z)}[\max(0, 1 + D(G(z)))]\Big)
%     \end{aligned}
% \end{equation}



% \section{DreamRefiner: efficient joint texture-geometry refinement}

% \subsection{Camera estimation and texture projection}

% \subsection{Efficient view-dependent object-aware diffusion prior}
% The pretrained 2D diffusion priors lack object awareness and lead to inconsistent optimization. To solve this problem, DreamCraft3D finetunes a pretrained diffusion model with the multi-view image renderings {x}, using DreamBooth, enabling the model to form a concept about the scene’s surrounding views. Though DreamBooth helps the pretrained diffusion model have global object awareness and benefit to consistent texture, it is inefficient to train DreamBooth. We propose to use Ip-adapter, a lightweight image prompt adaptation method with the decoupled cross-attention strategy for existing text-to-image diffusion models. Different from DreamBooth, Ip-adapter is training-free so it is much more efficient. 

% Give ip-adapter only the source image is ambiguous and lead to texture multi-head problem. To solve it, we condition generated multi-view renderings along with the source image. Similarly to DreamCraft3D, we use off-the-shelf upsampler to augment multi-view renderings before conditioning. In detail, we get the image embeddings of the ip adapter for all view images. During training, we select the ip adapter image embedding based on the location of the randomly sampled camera: if the camera is near front, we use the front source image. 


% \subsection{Joint texture-geometry refinement}

% \noindent\textbf{Camera and light augmentations.} We follow Magic3D to add random augmentations to the camera and light sampling for rendering the shaded images. Differently, we sample the point light location such that the angular distance from the random camera center location (w.r.t. the origin) is sampled with a random point light distance $r_\textnormal{cam} \sim (7.5, 10)$, and (b) we freeze the material augmentation unlike Dreamfusion and Magic3D, as we found it is bad for training convergence (c) In the coarse stage, we propose a fixed-random mixed camera pose strategy. Specifically, following the common practice of the current text-to-3D methods, random camera view sampling benefits scene optimization. However, Zero1-to-3 needs fixed camera intrinsic parameters. Therefore, we let half of the GPUs sample the camera distance from $\mathcal{U}(3.2,3.5)$, and the Field-of-View from $\mathcal{U}(10, 20)$, while the left GPUs are fixed to the default camera intrinsic.

% \noindent\textbf{iterative RGB and Normal rendering.} DreamCraft3D alternately renders normal maps $I_{normal}$ and RGB images $I_{RGB}$ as the input for diffusion guidance $I\_inp$ to enhance texture and geometry disentanglely. This strategy leads to finer geometry but geometry-texture misalignment because normal maps don't have RGB cues and hence leads to different optimization direction of geometry from texture. Our new strategy is to blend normal maps and RGB images with a random weight instead of only use normal maps as guidance input. 

% \begin{equation}
% \small
% \text{I\_inp} = 
% \begin{cases}
% I_{RGB} & \text{if } r < 0.5 \\
% \alpha \cdot I_{RGB} + (1 - \alpha) \cdot {I_{normal}} & \text{if } r \geq 0.5
% \end{cases}
% \end{equation}

% where $r \sim \text{Uniform}(0, 1)$ and $\alpha \sim \text{Uniform}(0, 0.5)$ is a random variable used to weight the RGB and normal components of the output when $r \geq 0.5$.

% \subsection{Loss functions}
% Since we adopt a training-free customized diffusion prior with multi-view renderings, we omit DreamBooth in DreamCraft3D~\cite{Sun2023DreamCraft3DH3}. Therefore, BSD is degraded to the standard VSD loss as below: 
% \begin{equation}
% \nabla_{\theta}\mathcal{L}_\textnormal{BSD}(\phi, g(\theta))=\mathbb{E}_{t, \bm{\epsilon}, c}[\omega(t)(\bm{\epsilon}_\textnormal{DreamBooth}(\bm{x}_{t};y,t,\{\tilde{x}\}_k,c)-\bm{\epsilon}_\textnormal{lora}(\bm{x}_{t};y,t,\{{x}\},c))\frac{\partial \bm{x}}{\partial \theta}].
% \label{eq:bsd}
% \end{equation}

% The total loss is:
% \begin{equation}
%         \mathcal{L}_{total} &= \mathcal{L}_{recon} + \mathcal{L}_{vsd}
% \end{equation}

